Harnessing Structures for Value-Based Planning and Reinforcement Learning

Value-based methods constitute a fundamental methodology in planning and deep reinforcement learning (RL). In this paper, we propose to exploit the underlying structures of the state-action value function, i.e., Q function, for both planning and deep RL. In particular, if the underlying system dynamics lead to some global structures of the Q function, one should be capable of inferring the function better by leveraging such structures. Specifically, we investigate the low-rank structure, which widely exists for big data matrices. We verify empirically the existence of low-rank Q functions in the context of control and deep RL tasks. As our key contribution, by leveraging Matrix Estimation (ME) techniques, we propose a general framework to exploit the underlying low-rank structure in Q functions. This leads to a more efficient planning procedure for classical control, and additionally, a simple scheme that can be applied to any value-based RL techniques to consistently achieve better performance on "low-rank" tasks. Extensive experiments on control tasks and Atari games confirm the efficacy of our approach. Code is available at https://github.com/YyzHarry/SV-RL.

==> introduction.tex <==
Value-based methods are widely used in control, planning and reinforcement learning tasks \citep{gorodetsky2018high, alora2016automated, mnih2015human, wang2015dueling}. To solve a Markov Decision Process (MDP), one common method is to use value iteration, which finds the optimal value function and the optimal policy.
This process can be done by iteratively computing and updating the state-action value function, represented by $Q(s,a)$~(i.e., the $Q$-value function).
In simple cases with small state and action spaces, value iteration can be ideal for efficient and accurate planning. However, for modern MDPs, the data that encodes the value function usually lies in thousands or millions of dimensions~\citep{gorodetsky2018high,gorodetsky2019continuous}, let alone continuous state space, such as images in deep reinforcement learning \citep{mnih2015human, tassa2018deepmind}. These practical constraints significantly hamper the efficiency and applicability of the vanilla value iteration.

However, the $Q$-value function is intrinsically induced by the underlying system dynamics. These dynamics are likely to possess some structured forms in various settings, such as being governed by partial differential equations. It is also possible that states and actions may contain latent features (e.g., similar states could have similar optimal actions). Thus, in those scenarios, it is reasonable to expect the structured dynamic to impose certain global \emph{structure} on the $Q$-value. 
% \red{Specifically, we look at low-rank structure in this paper. It exists widely in nature and we observe it in 43 out of 57 Atari games and all the 4 classical stochastic control tasks we experiment on.}
%This natural starting point raises an interesting suggestion: suppose that the $Q$-value function of the task under consideration indeed contains certain structures; then, instead of updating every $Q(s,a)$ for each iteration, we could update only a few of them for the current iteration and subsequently \emph{exploit} the interaction among all the $Q(s,a)$
%(i.e., the structure of the $Q$ function) to \emph{recover} the un-updated value. The ability to recover the value function with limited data can have a great impact on the efficiency, and hopefully, the exploitation of the structure also help to maintain the desired accuracy. 
%As such, the central questions are: (1) what kind of structures the value function may possess for certain tasks; (2) how to effectively exploit such a structure. 

To begin, we view the $Q$ function as a giant matrix, where each row represents a state, each column represents an action, and its $ij$-th entry represents the $Q$ value of the corresponding state-action pair. \red{Subsequently, we explore the global \emph{low-rank} structure of this matrix. Low-rank structure has been widely observed and exploited in modern big data analysis \citep{udell2019big}. As we will demonstrate empirically, this is also the case for our planning and RL scenarios: classical stochastic control tasks as well as most Atari games indeed contain the desired property.
}
% and leverage matrix estimation (ME) as our scheme to efficiently exploit the underlying structure. ME concerns with recovering a data matrix from potentially noisy or incomplete observations of its entries. When the data matrix is low-rank, exact or approximate recovery is theoretically guaranteed~\citep{chen2018harnessing,davenport2016overview}.
% We hypothesize that such a structure may arise for several reasons. The system dynamic itself may contain a low-dimensional representation, e.g., a partial differential equation, that eventually lead to a "low-dimensional" $Q$-value function. 
%Some past work has utilized this idea to do effective high-dimensional control via tensor decomposition \citep{gorodetsky2015efficient,gorodetsky2019continuous}.
% In addition, for certain tasks, states and actions may contain some latent features that determine the final behavior; for example, similar states could have a similar optimal actions. Such latent variable models on the rows and columns of a matrix often lead to approximate low-rank matrix \citep{udell2019big}.

\red{To exploit such low-rank structure, in this work, we propose a generic framework for both classical planning and modern deep RL. Our scheme leverages Matrix Estimation (ME), a theoretically guaranteed framework for recovering low-rank data matrix~\citep{chen2018harnessing,davenport2016overview}.}
In particular, for planning tasks in classical control problems, we propose Structured Value-based Planning (SVP). For the $Q$-value matrix of dimension $|\mathcal{S}|\times|\mathcal{A}|$, at each value iteration, SVP randomly updates a small portion of the $Q(s,a)$ and employs ME to reconstruct the remaining elements of the giant $Q$-value matrix. 
\red{We show that planning problems can greatly benefit from such a simple scheme, where much fewer samples can achieve almost the same policy as the optimal one.}

% While this clearly leads to more efficient planning, we further  We show that SVP can achieve comparable results to the optimal policy, with much more efficiency ; sampling 


For more advanced deep RL tasks, we extend our intuition and propose Structured Value-based Deep RL (SV-RL), applicable for any value-based methods such as DQN~\citep{mnih2015human}. Here, instead of the full $Q$-value matrix, SV-RL naturally focuses on the ``sub-matrix'' of the $Q$-value, corresponding to the sampled batch of states at current iteration.
\red{For each sampled $Q$-value matrix, we again apply ME to represent the deep $Q$ learning target in a structured way, which poses a low rank bias/regularization on this ``sub-matrix'' throughout the training process, and hence eventually the $Q$-network's prediction. Since learning a deep RL policy is often noisy with high variance, if the task itself possesses a low-rank property, this procedure will give a clear guidance during the learning process, after which a better policy can be anticipated.
We confirm that SV-RL indeed can consistently improve the performance of value-based methods on ``low-rank'' Atari games.
%We show that SV-RL can consistently improve the performance on vast majority of the Atari games, where the desired low-rank structures are indeed exist.
}
% To regularize and pose the low-rank structure for the eventually learned $Q$ function, Since learning a deep RL policy is often of high variance，this procedure hopefully guide the learning process to focus on the most important structure within the game.
% This procedure poses a low rank bias/regularization on the $Q$-network's prediction, and improves learning when the task itself possesses a low-rank property.
% We again leverage ME in SV-RL to exploit the structure within this sub-matrix.

%\red{another try:}
%In value-based deep reinforcement learning like DQN, the $Q$-value function matrix we are considering lies in minibatch during the training. At each state, the $Q$-network gives $Q(s,a)$ for all the possible actions for the agent in the form of a 1-d matrix, which accounts for 1 row of the $Q$-value function matrix in the minibatch. We intentionally samples part of the elements of the matrix and then do ME to recover, and use the recovered $Q$-values as the training data for the $Q$-network. 
%This procedure pose a low rank bias on the $Q$-network and improves learning when the task has low-rank properties. 

%We show that some classical stochastic control problems can greatly benefit from such a simple scheme, where much fewer samples can achieve almost the same policy as the optimal one. Drawing from the intuitions we develop, we extend our scheme to modern deep reinforcement learning. Since the states are now images, instead of viewing the $Q$-value functions as a matrix, which is no longer possible, we naturally focus on the "sub-matrix" resulted from the sampled batch. Before the SGD step, we view the current batch of states as a matrix: the rows are the states in the batch; the columns are the actions; and the matrix is populated by the associated $Q$-value from the $Q$-network. Instead of a simple SGD step on the batch of data, we exploit the structure among the states within the batch and leverage ME to form new targets for the SGD step. We provide extensive experimental validation on Atari games, demonstrating the efficacy of our scheme for many value-based deep reinforcement learning approaches.

We summarize our contributions as follows:
\begin{itemize}
    % \item We are the first to propose a complete framework that leverages matrix estimation as a general pipeline to exploit the {low-rank} structures, from planning to deep reinforcement learning.
    \item \red{We are the first to propose a framework that leverages matrix estimation as a general scheme to exploit the low-rank structures, from planning to deep reinforcement learning.}
    \item \red{We demonstrate the effectiveness of our approach on classical stochastic control tasks, where the low-rank structure allows for efficient planning with less computation.}
    \item 
    % We propose a simple scheme to exploit structures in deep reinforcement learning, applicable for any value-based techniques. Across a variety of methods, such as DQN, double DQN, and {dueling DQN}, experimental results  on all Atari games are well aligned with our arguments. 
    % showing consistent benefit for games possessing the desired structure. 
    \red{
    We extend our scheme to deep RL, which is naturally applicable for any value-based techniques. Across a variety of methods, such as DQN, double DQN, and dueling DQN, 
    experimental results on all Atari games show that SV-RL can consistently improve the performance of value-based methods, achieving higher scores for tasks when low-rank structures are confirmed to exist.}
    % are well aligned with our arguments. 
    % 43 out of 57 Atari games with good low-rank property show higher scores with our scheme, while the rest are similar or only slightly worse. 
\end{itemize}


% \vspace{-.15cm}
\begin{figure}[!t]
\centering
\subfigure[Vanilla value iteration]{
    \label{fig:toy_rank_vanilla}
    \includegraphics[width=0.24\textwidth]{figures/rank_vanilla.pdf}
}
\hspace{-1.7ex}
\subfigure[Vanilla value iteration]{
    \label{fig:toy_loss_vanilla}
    \includegraphics[width=0.24\textwidth]{figures/loss_vanilla.pdf}
}
\hspace{-1.7ex}
\subfigure[Online reconstruction]{
    \label{fig:toy_rank_me}
    \includegraphics[width=0.24\textwidth]{figures/rank_me.pdf}
}
\hspace{-1.7ex}
\subfigure[Online reconstruction]{
    \label{fig:toy_loss_me}
    \includegraphics[width=0.24\textwidth]{figures/loss_me.pdf}
}
\vspace{-.35cm}
\caption{The approximate rank and MSE of $Q^{(t)}$ during value iteration. (a) \& (b) use vanilla value iteration; (c) \& (d) use online reconstruction with only 50\% observed data each iteration.}
\label{fig:toy loss rank}
\vspace{-.35cm}
\end{figure}

